Sensitivity of the Hyper-Kamiokande experiment to neutrino oscillation parameters using acceleration neutrinos

This paper describes the analysis to estimate the sensitivity of the Hyper-Kamiokande experiment to long-baseline neutrino oscillation parameters using accelerator (anti)neutrinos. Results are presented for the CPV discovery sensitivity and precision measurements of the oscillation parameters $\delta_{CP}$, $\sin^2\theta_{23}$, $\Delta m^2_{32}$ and $\sin^2\theta_{13}$. With the assumed Hyper-Kamiokande running plan, a $5\sigma$ CPV discovery is possible in less than three years in the case of maximal CPV and known MO.In the absence of external constraints on the MO, considering the MO sensitivity of the Hyper-Kamiokande measurement using atmospheric neutrinos, the time for a CPV discovery could be estimated to be around six years. Using the nominal final exposure of $27 \times 10^{21}$ protons on target, corresponding to 10 years, with a ratio of 1:3 in neutrino to antineutrino beam mode, we expect to select approximately 10000 charged current, quasi-elastic-like, muon neutrino events, and a similar number of muon anti-neutrino events. In the electron (anti)neutrino appearance channels, we expect approximately 2000 charged current, quasi-elastic-like electron neutrino events and 800 electron antineutrino events. These larges event samples will allow Hyper-Kamiokande to exclude CP conservation at the $5\sigma$significance level for over 60% of the possible true values of $\delta_{CP}$.

==> Afteramble.tex <==
% Some commands might have to be renewed after \begin{document}, so can't be put in the Preamble
% Please put those commands here

% Renewing the autoref commands 
\renewcommand{\tableautorefname}{Tab.}
\renewcommand{\figureautorefname}{Fig.}
\renewcommand{\equationautorefname}{Eq.}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\renewcommand{\subsubsectionautorefname}{Sec.}

\renewcommand{\appendixautorefname}{App.}


==> Commands.tex <==

% Fit variables
\providecommand{\ssqthonethree}{\ensuremath{\sin^2\theta_{13}}\xspace}
\providecommand{\ssqthtwothree}{\ensuremath{\sin^2\theta_{23}}\xspace}
\providecommand{\ssqthonetwo}{\ensuremath{\sin^2\theta_{12}}\xspace}
\providecommand{\ssqthtwoonethree}{\ensuremath{\sin^2 2\theta_{13}}\xspace}

\providecommand{\poddet}{P\ensuremath{\emptyset}D\xspace}

%Upright CP on delta[cp]
%Note This also ensures "CP" the same size on the line $\deltacp$ compared to as an exponent $e^{i\delta}, => i.e. it doesn't get tiddly small when used in an exponent. 
\providecommand{\deltacp}{\ensuremath{\delta_{\scriptscriptstyle\mathrm{CP}}}\xspace}
\providecommand{\sindcp}{\ensuremath{\sin\deltacp}\xspace}
\providecommand{\cosdcp}{\ensuremath{\cos\deltacp}\xspace}
\providecommand{\dmsq}{\ensuremath{\Delta{}m^2}\xspace}
\providecommand{\dmsqtwothree}{\ensuremath{\Delta{}m^2_{32}}\xspace}
\providecommand{\dmsqonetwo}{\ensuremath{\Delta{}m^2_{21}}\xspace}
\providecommand{\dmsqonethree}{\ensuremath{\Delta{}m^2_{13}}\xspace}
\providecommand{\dmsqthreeone}{\ensuremath{\Delta{}m^2_{31}}\xspace}

\providecommand{\Enu}{\ensuremath{E_\nu}\xspace}

% FHC RHC
\providecommand{\fhc}{FHC\xspace}
\providecommand{\rhc}{RHC\xspace}
\providecommand{\fhcalt}{\ensuremath{\nu}-mode\xspace}
\providecommand{\rhcalt}{\ensuremath{\overline{\nu}}-mode\xspace}

\providecommand{\nova}{NOvA\xspace}
\providecommand{\minerva}{MINERvA\xspace}
\providecommand{\miniboone}{MiniBooNE\xspace}

%%2D fits
\providecommand{\appearance}{\deltacp vs \ssqthonethree\xspace}
\providecommand{\disappearance}{\dmsq vs \ssqthtwothree\xspace}
\providecommand{\main}{\deltacp vs \ssqthtwothree\xspace}

% Particle aliases
\providecommand{\nubar}{\ensuremath{\overline{\nu}}\xspace}
\providecommand{\nue}{\ensuremath{\nu_{e}}\xspace}
\providecommand{\numu}{\ensuremath{\nu_{\mu}}\xspace}
\providecommand{\nutau}{\ensuremath{\nu_{\tau}}\xspace}
\providecommand{\nueb}{\ensuremath{\nubar_{e}}\xspace}
\providecommand{\numub}{\ensuremath{\nubar_{\mu}}\xspace}
\providecommand{\nutaub}{\ensuremath{\nubar_{\tau}}\xspace}
\providecommand{\nub}{\nubar}
\providecommand{\nua}{\ensuremath{\nu_{\alpha}}\xspace}
\providecommand{\nuab}{\ensuremath{\nubar_{\alpha}}\xspace}

\def\thatm   {\ensuremath{\theta_{23}}\xspace}
\def\thsol   {\ensuremath{\theta_{12}}\xspace}
\def\thint   {\ensuremath{\theta_{13}}\xspace}

%% Generic parenthesis bar e.g. for nu/nubar
\newlength{\parenbarKernelHeight}
\providecommand{\parenbar}[1]{%
    \settoheight{\parenbarKernelHeight}{\ensuremath{#1}}%
    \addtolength{\parenbarKernelHeight}{0pt}
    \llap{\raisebox{\parenbarKernelHeight}{\scalebox{0.5}[0.5]{(}}}%
    \overline{#1}%
    \rlap{\raisebox{\parenbarKernelHeight}{\scalebox{0.5}[0.5]{)}}}%
    %\vphantom{#1}
}

\providecommand{\nuany}{\ensuremath{\hspace{0.5mm}\parenbar{\nu}}\xspace}
\providecommand{\numuany}{\ensuremath{\nuany_\mu}\xspace}
\providecommand{\nueany}{\ensuremath{\nuany_{e}}\xspace}

\providecommand{\pmu}{\ensuremath{p_\mu}\xspace}
\providecommand{\cosmu}{\ensuremath{\cos\theta_\mu}\xspace}

\providecommand{\CCzeropi}{CC$0\pi$\xspace}
\providecommand{\CConepi}{CC$1\pi$\xspace}
\providecommand{\CCother}{CC other\xspace}
\providecommand{\nueCConepi}{\nue\text{ CC}$1\pi^{+}$\xspace}
\providecommand*{\pbar}[1]{\accentset{(-)}{#1}\xspace}

\providecommand{\rmu}{1R$\mu$\xspace}
\providecommand{\re}{1R$e$\xspace}
\providecommand{\rede}{1R$e$1d$e$\xspace}
\providecommand{\de}{d$e$}

\providecommand{\oscprob}[2]{\ensuremath{P\left(\nu_{#1}\rightarrow\nu_{#2}\right)}\xspace}
\providecommand{\oscprobb}[2]{\ensuremath{P\left(\overline{\nu}_{#1}\rightarrow\overline{\nu}_{#2}\right)}\xspace}
\providecommand{\oscprobshort}[2]{\ensuremath{P_{#1 #2}}\xspace}
\providecommand{\oscprobbshort}[2]{\ensuremath{P_{\overline{#1}\overline{#2}}}\xspace}

\providecommand{\etal}{\emph{et al.}\xspace}

\renewcommand{\labelitemi}{\textbullet}

\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}
\renewcommand{\topfraction}{0.85}
\renewcommand{\bottomfraction}{0.85}
\renewcommand{\textfraction}{0.15}
\renewcommand{\floatpagefraction}{0.7}


==> Preamble.tex <==
\RequirePackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\RequirePackage{graphicx}
\RequirePackage{mathptmx}
\RequirePackage{mathtools}
\RequirePackage{amsmath,amssymb}
\RequirePackage{multirow}
\RequirePackage{xspace}
\RequirePackage{placeins}
\RequirePackage{appendix}

\usepackage[normalem]{ulem}

\usepackage{braket}

\usepackage{hhline}
\usepackage{gensymb}
\usepackage{subcaption}

\usepackage{caption}
\captionsetup[table]{name=Tab.}
\captionsetup[figure]{name=Fig.}

\usepackage{enumitem}

%\usepackage{cite}

\RequirePackage{flushend}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=blue,      
    urlcolor=blue,
    pdftitle={HyperKamiokande sensitivity to long baseline neutrino oscillations},
    }

\emergencystretch=1em

\journalname{Eur. Phys. J. C}

%\input{Commands.tex}
%new from me
%\usepackage{amssymb,amsmath,amstext,amsthm,amsfonts}
\usepackage{amssymb,amsmath,amstext,amsfonts}
\usepackage{tikz}
\usepackage{xcolor}
\usepackage{hyperref}
\usepackage{comment}
%\usepackage{subfigure}
\usepackage{float}
\usepackage{url}
\usepackage{multirow}
%\usepackage{todonotes}
\usepackage{soul}
\usepackage{cuted}
%\usepackage{multicol}
\usepackage{flushend}
\usepackage{dblfloatfix}
\usepackage[english]{babel}
\usepackage{gensymb}
%\babelhyphenation[british]{def–i–ni–tion}
%\babelhyphenation[british]{ma-trix}
\usepackage{multicol}
\usepackage{orcidlink}%
\newcommand\barparen[1]{\overset{(-)}{#1}}
